A Secure, Confidential, and Verifiable Decision Support System

Decision support systems are increasingly adopted to automate decision-making processes across industries, organizations, and governments. Decision support demands data privacy, integrity, and availability while ensuring customization, security, and verifiability of the decision process. Existing solutions fail to guarantee those properties altogether. To overcome this limitation, we propose SPARTA, an approach based on Trusted Execution Environments (TEEs) that automates decision processes. To guarantee privacy, integrity, and availability, SPARTA employs efficient cryptographic techniques on notarized data with access mediated through user-defined access policies. Our solution allows users to define decision rules, which are translated to certified software objects deployed within TEEs, thereby guaranteeing customization, verifiability, and security of the process. With experiments run on public benchmarks and synthetic data, we show our approach is scalable and adds limited overhead compared to non-cryptographically secured solutions.

==> addon/commands-for-inline-referenceable-objects-with-counter.tex <==
%%%% A command for inline requirements. This one alters the counter from arabic to arabic with an "R" prefix, boldface
%%%% ----------------------------------------------------------------
\newcounter{req}
% When defining a new counter, say ``req'', then command ``\thereq'' is generated automatically. Hence the need for a ``\renewcommand''
\renewcommand{\thereq}{R\arabic{req}}
\newcommand\Req[0]{%
	\refstepcounter{req}%
	\textbf{\thereq}}
% For the references with the cleveref package
\RequirePackage{cleveref}
\crefname{req}{Req.}{Reqs.}
\Crefname{req}{Requirement}{Requirements}
%%%% Usage example:
%%%%   Our work firstly pursues the objective of preserving \Req\label{req:secrecy} in process data treatment.
%%%%   [..]
%%%%   Therefore, our approach aims to yield \cref{req:secrecy}






%%%%% A command for inline question list. This one alters the counter from arabic to arabic with an "R" prefix, boldface
%%%%% ----------------------------------------------------------------
\RequirePackage[inline]{enumitem}
%%
\def\questiprefix{Q}
\def\questinum{\questiprefix\arabic*}
%% https://tex.stackexchange.com/questions/410585/cleveref-format-for-enumerate    
\newlist{questiilist}{enumerate*}{1}  % create a new enumerate-like environment
\setlist[questiilist,1]{label={(\textbf{\questinum})},itemjoin={~},before={},ref=\questinum}
%% For the references with the cleveref package
\RequirePackage{cleveref}
\crefname{questiilisti}{question}{questions} % questiilist*i* to indicate level 1 (automatically assigned)
\Crefname{questiilisti}{Question}{Questions}
%%%%% Usage example:
%%%%%   \begin{questiilist}
%%%%%   	\item Monitor parties must [...] \label{qst:trustworthiness}
%%%%%    [..]
%%%%%   \end{questiilist}
%%%%%   [..]
%%%%%   articles for each of \cref{qst:trustworthiness,qst:noleakage,qst:nopeeking,qst:operativeness}
%%%%%   [..]
%%%%%   \ref{qst:trustworthiness} 
%%%%%   Therefore, our approach aims to yield \cref{obj:secrecy}

==> code/feel-formulas.txt.tex <==



avgOnTimeDeliv
filteredCarriers: 
	Carrier[ISOCompliant = true], 
avgOnTimeDeliveryRate: 
	mean(filteredCarriers.OnTimeDeliveryRate)

meanAge
filteredPatients: 
	Patient[ConsentFormSigned = true and 
	contains(FamilyMedicalHistory, "Heart Disease") 
	and (Age <= 38 or (Age > 40 and 
	contains(PreExistingConditions, "Diabetes"))) and 
	contains(PreviousVaccinations, "COVID-19")], 
meanAge: mean(filteredPatients.Age)

sumAge
filteredPatients: 
	Patient[ConsentFormSigned = true], 
sumAge: sum(filteredPatients.Age)


patients: Patient[contains(FamilyMedicalHistory, 'Heart Disease') and ConsentFormSigned = true], avgAge: mean(patients.Age)

{ totalAvailableVaccines: sum(medicalHub.QuantityAvailable), 
  activeCenters: vaccinationCenters[VaccinationProgress > 0],
  totalDailyVaccinations: sum(activeCenters.VaccinationProgress),
  stockCoverageDays: totalAvailableVaccines / totalDailyVaccinations }.stockCoverageDays
